Fix Fairness, Don't Ruin Accuracy: Performance Aware Fairness Repair using AutoML

Machine learning (ML) is increasingly being used in critical decision-making software, but incidents have raised questions about the fairness of ML predictions. To address this issue, new tools and methods are needed to mitigate bias in ML-based software. Previous studies have proposed bias mitigation algorithms that only work in specific situations and often result in a loss of accuracy. Our proposed solution is a novel approach that utilizes automated machine learning (AutoML) techniques to mitigate bias. Our approach includes two key innovations: a novel optimization function and a fairness-aware search space. By improving the default optimization function of AutoML and incorporating fairness objectives, we are able to mitigate bias with little to no loss of accuracy. Additionally, we propose a fairness-aware search space pruning method for AutoML to reduce computational cost and repair time. Our approach, built on the state-of-the-art Auto-Sklearn tool, is designed to reduce bias in real-world scenarios. In order to demonstrate the effectiveness of our approach, we evaluated our approach on four fairness problems and 16 different ML models, and our results show a significant improvement over the baseline and existing bias mitigation techniques. Our approach, Fair-AutoML, successfully repaired 60 out of 64 buggy cases, while existing bias mitigation techniques only repaired up to 44 out of 64 cases.

==> evaluation/overall.tex <==
\begin{table*}[ht]
\centering
\caption{FairAutoML}
\setlength{\tabcolsep}{0.9pt}
\scriptsize
\begin{tabular}{|c|c|c|
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFFC9E}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |c|c|
>{\columncolor[HTML]{FFCCC9}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFCE93}}c |
>{\columncolor[HTML]{FFFC9E}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |
>{\columncolor[HTML]{9AFF99}}c |}
\hline
                           & Model                  & Metric & BL    & T1    & T2    & T3    & T4    & AS    & R     & D     & A     & E     & C     & O     & Model                  & Metric & BL    & T1    & T2    & T3    & T4    & AS    & R     & D     & A     & E     & C     & O     \\ \hline
                                  &                        & Acc    & 0.844 & 0.846 & 0.838 & 0.852 & 0.852 & 0.859 & 0.851 & 0.845 & 0.775 & 0.835 & 0.832 & 0.794 &                        & Acc    & 0.849 & 0.845 & 0.827 & 0.844 & 0.832 & 0.850 & 0.790 & 0.791 & 0.725 & 0.790 & 0.789 & 0.786 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 0.563 & 0.450 & 0.470 & 0.455 & 0.437 & 0.512 & 0.234 & 0.588 & 0.356 & 0.279 & 0.431 & 0.126 &                        & DI     & 0.620 & 0.562 & 0.533 & 0.504 & 0.454 & 0.583 & 0.096 & 0.339 & 0.375 & 0.290 & 0.330 & 0.347 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.099 & 0.073 & 0.055 & 0.075 & 0.071 & 0.084 & 0.045 & 0.105 & 0.014 & 0.054 & 0.072 & 0.046 &                        & SPD    & 0.100 & 0.092 & 0.076 & 0.083 & 0.067 & 0.097 & 0.009 & 0.026 & 0.015 & 0.023 & 0.025 & 0.033 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.045 & 0.032 & 0.026 & 0.023 & 0.026 & 0.045 & 0.059 & 0.058 & 0.020 & 0.007 & 0.036 & 0.067 &                        & EOD    & 0.062 & 0.059 & 0.051 & 0.042 & 0.028 & 0.088 & 0.015 & 0.016 & 0.013 & 0.005 & 0.012 & 0.013 \\ \cline{3-15} \cline{17-29} 
                                  & \multirow{-5}{*}{RF}   & AOD    & 0.044 & 0.026 & 0.019 & 0.020 & 0.018 & 0.035 & 0.049 & 0.052 & 0.010 & 0.003 & 0.006 & 0.039 & \multirow{-5}{*}{LRG}  & AOD    & 0.084 & 0.045 & 0.039 & 0.034 & 0.023 & 0.062 & 0.009 & 0.010 & 0.007 & 0.002 & 0.005 & 0.010 \\ \cline{2-29} 
                                  &                        & Acc    & 0.870 & 0.848 & 0.805 & 0.848 & 0.844 & 0.869 & 0.865 & 0.848 & 0.659 & 0.831 & 0.831 & 0.810 &                        & Acc    & 0.864 & 0.857 & 0.823 & 0.867 & 0.861 & 0.874 & 0.857 & 0.852 & 0.805 & 0.844 & 0.840 & 0.803 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 0.604 & 0.401 & 0.300 & 0.452 & 0.443 & 0.621 & 0.210 & 0.677 & 0.305 & 0.258 & 0.466 & 0.132 &                        & DI     & 0.573 & 0.425 & 0.387 & 0.441 & 0.439 & 0.591 & 0.169 & 0.529 & 0.423 & 0.328 & 0.390 & 0.117 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.102 & 0.063 & 0.022 & 0.073 & 0.058 & 0.102 & 0.042 & 0.122 & 0.015 & 0.048 & 0.075 & 0.045 &                        & SPD    & 0.088 & 0.069 & 0.038 & 0.069 & 0.069 & 0.098 & 0.030 & 0.083 & 0.065 & 0.053 & 0.057 & 0.040 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.056 & 0.044 & 0.023 & 0.029 & 0.019 & 0.080 & 0.085 & 0.115 & 0.007 & 0.006 & 0.012 & 0.069 &                        & EOD    & 0.046 & 0.021 & 0.026 & 0.026 & 0.025 & 0.065 & 0.047 & 0.046 & 0.109 & 0.006 & 0.034 & 0.054 \\ \cline{3-15} \cline{17-29} 
\multirow{-10}{*}{\rotatebox[origin=c]{90}{Adult Census}}   & \multirow{-5}{*}{XGB}  & AOD    & 0.076 & 0.026 & 0.013 & 0.021 & 0.012 & 0.057 & 0.060 & 0.085 & 0.004 & 0.002 & 0.013 & 0.038 & \multirow{-5}{*}{GBC}  & AOD    & 0.066 & 0.015 & 0.015 & 0.016 & 0.017 & 0.047 & 0.034 & 0.034 & 0.072 & 0.002 & 0.012 & 0.038 \\ \hline
                                  &                        & Acc    & 0.889 & 0.895 & 0.884 & 0.906 & 0.899 & 0.919 & 0.898 & 0.893 & 0.889 & 0.873 & 0.893 & 0.824 &                        & Acc    & 0.906 & 0.905 & 0.898 & 0.907 & 0.909 & 0.910 & 0.908 & 0.826 & 0.887 & 0.832 & 0.834 & 0.763 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 0.763 & 0.561 & 0.439 & 0.632 & 0.625 & 0.663 & 0.453 & 0.733 & 0.763 & 0.351 & 0.603 & 0.439 &                        & DI     & 0.704 & 0.546 & 0.468 & 0.538 & 0.607 & 0.581 & 0.392 & 0.083 & 0.646 & 0.233 & 0.124 & 0.099 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.038 & 0.062 & 0.038 & 0.090 & 0.070 & 0.096 & 0.032 & 0.077 & 0.038 & 0.038 & 0.058 & 0.046 &                        & SPD    & 0.106 & 0.074 & 0.055 & 0.079 & 0.085 & 0.088 & 0.053 & 0.019 & 0.046 & 0.051 & 0.026 & 0.034 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.052 & 0.061 & 0.054 & 0.061 & 0.062 & 0.053 & 0.096 & 0.080 & 0.052 & 0.006 & 0.039 & 0.065 &                        & EOD    & 0.054 & 0.060 & 0.071 & 0.051 & 0.041 & 0.062 & 0.082 & 0.137 & 0.064 & 0.011 & 0.027 & 0.059 \\ \cline{3-15} \cline{17-29} 
                                  & \multirow{-5}{*}{RF}   & AOD    & 0.026 & 0.039 & 0.033 & 0.040 & 0.039 & 0.039 & 0.057 & 0.051 & 0.026 & 0.003 & 0.023 & 0.037 & \multirow{-5}{*}{XGB2} & AOD    & 0.058 & 0.034 & 0.040 & 0.031 & 0.031 & 0.041 & 0.064 & 0.096 & 0.033 & 0.004 & 0.026 & 0.038 \\ \cline{2-29} 
                                  &                        & Acc    & 0.882 & 0.902 & 0.905 & 0.911 & 0.904 & 0.910 & 0.896 & 0.884 & 0.882 & 0.846 & 0.884 & 0.886 &                        & Acc    & 0.907 & 0.903 & 0.899 & 0.920 & 0.917 & 0.900 & 0.907 & 0.841 & 0.890 & 0.849 & 0.847 & 0.803 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 3.279 & 0.600 & 0.350 & 0.584 & 0.606 & 0.653 & 0.476 & 0.524 & 3.279 & 0.258 & 0.563 & 0.515 &                        & DI     & 0.610 & 0.600 & 0.541 & 0.599 & 0.624 & 0.610 & 0.278 & 0.166 & 0.646 & 0.254 & 0.063 & 0.111 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.612 & 0.084 & 0.045 & 0.084 & 0.087 & 0.096 & 0.065 & 0.087 & 0.612 & 0.045 & 0.085 & 0.047 &                        & SPD    & 0.085 & 0.087 & 0.057 & 0.087 & 0.094 & 0.083 & 0.034 & 0.034 & 0.040 & 0.049 & 0.012 & 0.033 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.664 & 0.043 & 0.066 & 0.053 & 0.047 & 0.063 & 0.113 & 0.066 & 0.664 & 0.010 & 0.034 & 0.076 &                        & EOD    & 0.047 & 0.064 & 0.073 & 0.048 & 0.052 & 0.061 & 0.069 & 0.214 & 0.065 & 0.011 & 0.072 & 0.079 \\ \cline{3-15} \cline{17-29} 
\multirow{-10}{*}{\rotatebox[origin=c]{90}{Bank Marketing}} & \multirow{-5}{*}{XGB1} & AOD    & 0.614 & 0.031 & 0.034 & 0.031 & 0.029 & 0.047 & 0.085 & 0.037 & 0.614 & 0.004 & 0.027 & 0.032 & \multirow{-5}{*}{GBC}  & AOD    & 0.061 & 0.047 & 0.038 & 0.034 & 0.036 & 0.045 & 0.045 & 0.141 & 0.036 & 0.004 & 0.057 & 0.054 \\ \hline
                                  &                        & Acc    & 0.771 & 0.842 & 0.830 & 0.820 & 0.793 & 0.835 & 0.741 & 0.750 & 0.742 & 0.734 & 0.250 & 0.311 &                        & Acc    & 0.748 & 0.756 & 0.762 & 0.786 & 0.775 & 0.789 & 0.732 & 0.736 & 0.726 & 0.703 & 0.270 & 0.542 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 0.115 & 0.090 & 0.073 & 0.078 & 0.052 & 0.097 & 0.058 & 0.085 & 0.093 & 0.029 & 0.313 & 0.000 &                        & DI     & 0.232 & 0.064 & 0.054 & 0.063 & 0.108 & 0.147 & 0.141 & 0.172 & 0.089 & 0.031 & 0.598 & 0.002 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.090 & 0.068 & 0.055 & 0.060 & 0.041 & 0.072 & 0.046 & 0.066 & 0.071 & 0.023 & 0.066 & 0.001 &                        & SPD    & 0.170 & 0.050 & 0.042 & 0.051 & 0.080 & 0.106 & 0.105 & 0.127 & 0.073 & 0.024 & 0.101 & 0.005 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.095 & 0.028 & 0.028 & 0.026 & 0.024 & 0.035 & 0.029 & 0.041 & 0.072 & 0.018 & 0.040 & 0.002 &                        & EOD    & 0.181 & 0.040 & 0.031 & 0.029 & 0.039 & 0.064 & 0.086 & 0.086 & 0.050 & 0.018 & 0.077 & 0.007 \\ \cline{3-15} \cline{17-29} 
                                  & \multirow{-5}{*}{RF}   & AOD    & 0.060 & 0.049 & 0.045 & 0.049 & 0.038 & 0.042 & 0.069 & 0.067 & 0.082 & 0.009 & 0.066 & 0.001 & \multirow{-5}{*}{SVC}  & AOD    & 0.092 & 0.047 & 0.041 & 0.049 & 0.068 & 0.090 & 0.127 & 0.126 & 0.091 & 0.014 & 0.114 & 0.004 \\ \cline{2-29} 
                                  &                        & Acc    & 0.727 & 0.812 & 0.807 & 0.801 & 0.821 & 0.844 & 0.718 & 0.720 & 0.722 & 0.703 & 0.280 & 0.303 &                        & Acc    & 0.754 & 0.797 & 0.816 & 0.826 & 0.817 & 0.826 & 0.720 & 0.724 & 0.721 & 0.712 & 0.274 & 0.295 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 0.106 & 0.070 & 0.084 & 0.076 & 0.075 & 0.150 & 0.065 & 0.083 & 0.087 & 0.025 & 0.213 & 0.241 &                        & DI     & 0.100 & 0.070 & 0.084 & 0.091 & 0.087 & 0.118 & 0.095 & 0.119 & 0.102 & 0.016 & 0.373 & 0.000 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.094 & 0.053 & 0.061 & 0.057 & 0.055 & 0.108 & 0.047 & 0.059 & 0.073 & 0.018 & 0.059 & 0.016 &                        & SPD    & 0.073 & 0.054 & 0.062 & 0.070 & 0.068 & 0.090 & 0.077 & 0.096 & 0.083 & 0.013 & 0.109 & 0.000 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.103 & 0.038 & 0.038 & 0.031 & 0.032 & 0.038 & 0.039 & 0.039 & 0.049 & 0.013 & 0.039 & 0.014 &                        & EOD    & 0.071 & 0.030 & 0.035 & 0.026 & 0.031 & 0.040 & 0.063 & 0.063 & 0.079 & 0.014 & 0.085 & 0.000 \\ \cline{3-15} \cline{17-29} 
\multirow{-10}{*}{\rotatebox[origin=c]{90}{German Credit}}  & \multirow{-5}{*}{XGB}  & AOD    & 0.050 & 0.042 & 0.059 & 0.046 & 0.046 & 0.068 & 0.068 & 0.068 & 0.095 & 0.011 & 0.068 & 0.021 & \multirow{-5}{*}{KNN}  & AOD    & 0.054 & 0.056 & 0.044 & 0.055 & 0.048 & 0.076 & 0.105 & 0.105 & 0.096 & 0.012 & 0.108 & 0.000 \\ \hline
                                  &                        & Acc    & 0.813 & 0.827 & 0.767 & 0.777 & 0.775 & 0.871 & 0.647 & 0.792 & 0.656 & 0.634 & 0.783 & 0.635 &                        & Acc    & 0.811 & 0.780 & 0.795 & 0.748 & 0.768 & 0.876 & 0.671 & 0.796 & 0.656 & 0.622 & 0.792 & 0.646 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 2.281 & 1.448 & 1.166 & 1.081 & 0.985 & 2.225 & 1.855 & 2.231 & 0.416 & 0.367 & 2.533 & 0.088 &                        & DI     & 2.040 & 0.957 & 1.029 & 0.826 & 1.089 & 1.991 & 1.698 & 2.046 & 0.537 & 0.315 & 2.282 & 0.092 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.693 & 0.440 & 0.330 & 0.343 & 0.300 & 0.688 & 0.539 & 0.658 & 0.103 & 0.092 & 0.917 & 0.043 &                        & SPD    & 0.684 & 0.339 & 0.351 & 0.292 & 0.335 & 0.698 & 0.533 & 0.666 & 0.125 & 0.104 & 0.873 & 0.043 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.521 & 0.278 & 0.238 & 0.160 & 0.127 & 0.538 & 0.674 & 0.605 & 0.086 & 0.040 & 0.762 & 0.065 &                        & EOD    & 0.507 & 0.187 & 0.192 & 0.135 & 0.271 & 0.449 & 0.645 & 0.566 & 0.088 & 0.045 & 0.698 & 0.081 \\ \cline{3-15} \cline{17-29} 
                                  & \multirow{-5}{*}{RF}   & AOD    & 0.644 & 0.186 & 0.147 & 0.108 & 0.072 & 0.421 & 0.573 & 0.511 & 0.061 & 0.026 & 0.860 & 0.159 & \multirow{-5}{*}{GBC}  & AOD    & 0.593 & 0.187 & 0.116 & 0.081 & 0.118 & 0.417 & 0.550 & 0.512 & 0.059 & 0.025 & 0.789 & 0.184 \\ \cline{2-29} 
                                  &                        & Acc    & 0.799 & 0.802 & 0.765 & 0.747 & 0.728 & 0.826 & 0.639 & 0.813 & 0.665 & 0.572 & 0.802 & 0.646 &                        & Acc    & 0.805 & 0.781 & 0.770 & 0.792 & 0.765 & 0.847 & 0.676 & 0.799 & 0.644 & 0.648 & 0.796 & 0.646 \\ \cline{3-15} \cline{17-29} 
                                  &                        & DI     & 2.588 & 1.735 & 1.446 & 1.192 & 0.898 & 2.457 & 2.056 & 2.439 & 0.580 & 0.193 & 2.499 & 0.096 &                        & DI     & 2.260 & 0.998 & 1.217 & 1.216 & 1.143 & 2.418 & 1.589 & 2.057 & 0.379 & 0.449 & 2.175 & 0.088 \\ \cline{3-15} \cline{17-29} 
                                  &                        & SPD    & 0.825 & 0.575 & 0.423 & 0.353 & 0.229 & 0.762 & 0.688 & 0.818 & 0.161 & 0.081 & 0.875 & 0.040 &                        & SPD    & 0.683 & 0.371 & 0.295 & 0.417 & 0.366 & 0.694 & 0.481 & 0.618 & 0.096 & 0.116 & 0.720 & 0.041 \\ \cline{3-15} \cline{17-29} 
                                  &                        & EOD    & 0.724 & 0.473 & 0.373 & 0.235 & 0.229 & 0.673 & 0.736 & 0.715 & 0.077 & 0.065 & 0.732 & 0.101 &                        & EOD    & 0.521 & 0.194 & 0.192 & 0.256 & 0.264 & 0.600 & 0.592 & 0.527 & 0.049 & 0.048 & 0.591 & 0.098 \\ \cline{3-15} \cline{17-29} 
\multirow{-10}{*}{\rotatebox[origin=c]{90}{Titanic}}        & \multirow{-5}{*}{LRG}  & AOD    & 0.760 & 0.389 & 0.283 & 0.167 & 0.094 & 0.593 & 0.692 & 0.693 & 0.053 & 0.045 & 0.785 & 0.185 & \multirow{-5}{*}{XGB}  & AOD    & 0.609 & 0.143 & 0.134 & 0.205 & 0.161 & 0.473 & 0.493 & 0.435 & 0.050 & 0.024 & 0.573 & 0.187 \\ \hline
\end{tabular}%%
\label{tbl:overall}
\centering

\scriptsize \* RF: Random Forest, XGB: XGBoost, LRG: Logistic Regression, SVC: Support Vector Classifier, KNN: K-Nearest Neighbors,  GBC: Gradient Boosting Classifier. T1, T2, T3, T4: \fairautoml with different objective functions, AS: \as, R: Reweighing, D: DI Remover, A: Adversarial Debiasing, E: Equalized Odds, C: Calibrated Equalized Odds, O: Reject Option Classification.
\end{table*}

==> evaluation/temp.tex <==
% \begin{table*}[t]
% \centering
% \caption{Trade-off assessment results of \fairautoml, \as, and mitigation techniques}
% \setlength{\tabcolsep}{0.1pt}
% \footnotesize
% \fontsize{8.7}{8.7}
% \selectfont
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
%                                   & \textbf{}           & \textbf{T1}                                        & \textbf{T2}                                                 & \textbf{T3}                                                 & \textbf{T4}                                                 & \multicolumn{1}{c|}{\textbf{AS}}       & \multicolumn{1}{c|}{\textbf{R}}        & \multicolumn{1}{c|}{\textbf{D}}        & \multicolumn{1}{c|}{\textbf{A}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c|}{\textbf{C}}        & \textbf{O}                    & \textbf{}           & \multicolumn{1}{c|}{\textbf{T1}}       & \multicolumn{1}{c|}{\textbf{T2}}       & \multicolumn{1}{c|}{\textbf{T3}}       & \multicolumn{1}{c|}{\textbf{T4}}       & \multicolumn{1}{c|}{\textbf{AS}}       & \multicolumn{1}{c|}{\textbf{R}}        & \multicolumn{1}{c|}{\textbf{D}}        & \multicolumn{1}{c|}{\textbf{A}}        & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c|}{\textbf{C}} & \textbf{O}                    \\ \hline
%                                   &                     & \cellcolor[HTML]{D8FFD7}0.010                                              & \cellcolor[HTML]{D8FFD7}0.001                                                       & \cellcolor[HTML]{D8FFD7}0.005                                                       & \cellcolor[HTML]{D8FFD7}-0.003                                                      & \cellcolor[HTML]{D8FFD7}0.016                                  & \cellcolor[HTML]{D8FFD7}0.009                                  & \cellcolor[HTML]{D8FFD7}0.004                                  & \cellcolor[HTML]{D8FFD7}-0.066                          & \cellcolor[HTML]{D8FFD7}-0.006                          & \cellcolor[HTML]{D8FFD7}-0.010                                 & \cellcolor[HTML]{D8FFD7}-0.047                        &                     & \cellcolor[HTML]{D8FFD7}-0.013                                 & \cellcolor[HTML]{D8FFD7}-0.022                                 & \cellcolor[HTML]{D8FFD7}-0.009                                 & \cellcolor[HTML]{D8FFD7}-0.032                                 & \cellcolor[HTML]{D8FFD7}-0.001                                 & \cellcolor[HTML]{D8FFD7}-0.056                                 & \cellcolor[HTML]{D8FFD7}-0.055                                 & \cellcolor[HTML]{D8FFD7}-0.121                                 & \cellcolor[HTML]{D8FFD7}-0.057                          & \cellcolor[HTML]{D8FFD7}-0.057                          & \cellcolor[HTML]{D8FFD7}-0.061                        \\ 
%                                   &                     & \cellcolor[HTML]{ECF4FF}\textbf{0.096}             & \cellcolor[HTML]{ECF4FF}\textbf{0.011}                      & \cellcolor[HTML]{ECF4FF}\textbf{0.118}                      & \cellcolor[HTML]{ECF4FF}0.095                               & \cellcolor[HTML]{ECF4FF}\textbf{0.058} & \cellcolor[HTML]{ECF4FF}\textbf{0.337} & \cellcolor[HTML]{ECF4FF}inv            & \cellcolor[HTML]{ECF4FF}0.215   & \cellcolor[HTML]{ECF4FF}0.292   & \cellcolor[HTML]{ECF4FF}0.140          & \cellcolor[HTML]{ECF4FF}0.445 &                     & \cellcolor[HTML]{ECF4FF}0.190          & \cellcolor[HTML]{ECF4FF}0.410          & \cellcolor[HTML]{ECF4FF}0.212          & \cellcolor[HTML]{ECF4FF}0.179          & \cellcolor[HTML]{ECF4FF}0.040          & \cellcolor[HTML]{ECF4FF}0.569          & \cellcolor[HTML]{ECF4FF}0.326          & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}0.375   & \cellcolor[HTML]{ECF4FF}0.335   & \cellcolor[HTML]{ECF4FF}0.318 \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}\textbf{0.023}             & \cellcolor[HTML]{FFFFC7}\textbf{0.024}                      & \cellcolor[HTML]{FFFFC7}\textbf{0.038}                      & \cellcolor[HTML]{FFFFC7}0.048                               & \cellcolor[HTML]{FFFFC7}\textbf{0.016} & \cellcolor[HTML]{FFFFC7}\textbf{0.055} & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}0.086   & \cellcolor[HTML]{FFFFC7}0.047   & \cellcolor[HTML]{FFFFC7}0.028          & \cellcolor[HTML]{FFFFC7}0.055 &                     & \cellcolor[HTML]{FFFFC7}0.054          & \cellcolor[HTML]{FFFFC7}0.075          & \cellcolor[HTML]{FFFFC7}0.029          & \cellcolor[HTML]{FFFFC7}0.059          & \cellcolor[HTML]{FFFFC7}0.005          & \cellcolor[HTML]{FFFFC7}0.097          & \cellcolor[HTML]{FFFFC7}0.079          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.083   & \cellcolor[HTML]{FFFFC7}0.081   & \cellcolor[HTML]{FFFFC7}0.072 \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}\textbf{0.019}             & \cellcolor[HTML]{EFEFEF}inv                                 & \cellcolor[HTML]{EFEFEF}\textbf{0.014}                      & \cellcolor[HTML]{EFEFEF}0.020                               & \cellcolor[HTML]{EFEFEF}\textbf{0.008} & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}0.041   & \cellcolor[HTML]{EFEFEF}0.012          & \cellcolor[HTML]{EFEFEF}lose  &                     & \cellcolor[HTML]{EFEFEF}0.048          & \cellcolor[HTML]{EFEFEF}0.020          & \cellcolor[HTML]{EFEFEF}0.044          & \cellcolor[HTML]{EFEFEF}0.049          & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}0.057          & \cellcolor[HTML]{EFEFEF}0.056          & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}0.067   & \cellcolor[HTML]{EFEFEF}0.060   & \cellcolor[HTML]{EFEFEF}0.059 \\
%                                   & \multirow{-5}{*}{F} & \cellcolor[HTML]{FFE2E1}\textbf{0.028}             & \cellcolor[HTML]{FFE2E1}inv                                 & \cellcolor[HTML]{FFE2E1}\textbf{0.030}                      & \cellcolor[HTML]{FFE2E1}0.035                               & \cellcolor[HTML]{FFE2E1}\textbf{0.021} & \cellcolor[HTML]{FFE2E1}\textbf{0.005} & \cellcolor[HTML]{FFE2E1}\textbf{0.001} & \cellcolor[HTML]{FFE2E1}0.044   & \cellcolor[HTML]{FFE2E1}0.051   & \cellcolor[HTML]{FFE2E1}0.048          & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{L} & \cellcolor[HTML]{FFE2E1}0.085          & \cellcolor[HTML]{FFE2E1}0.075          & \cellcolor[HTML]{FFE2E1}0.079          & \cellcolor[HTML]{FFE2E1}0.089          & \cellcolor[HTML]{FFE2E1}0.039          & \cellcolor[HTML]{FFE2E1}0.096          & \cellcolor[HTML]{FFE2E1}0.094          & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.103   & \cellcolor[HTML]{FFE2E1}0.100   & \cellcolor[HTML]{FFE2E1}0.095 \\ \cline{2-25} 
%                                   &                     & \cellcolor[HTML]{D8FFD7}-0.019                                             & \cellcolor[HTML]{D8FFD7}-0.052                                                      & \cellcolor[HTML]{D8FFD7}-0.017                                                      & \cellcolor[HTML]{D8FFD7}-0.015                                                      & \cellcolor[HTML]{D8FFD7}-0.001                                 & \cellcolor[HTML]{D8FFD7}-0.001                                 & \cellcolor[HTML]{D8FFD7}-0.018                                 & \cellcolor[HTML]{D8FFD7}-0.207                          & \cellcolor[HTML]{D8FFD7}-0.035                          & \cellcolor[HTML]{D8FFD7}-0.035                                 & \cellcolor[HTML]{D8FFD7}-0.056                        &                     & \cellcolor[HTML]{D8FFD7}-0.023                                 & \cellcolor[HTML]{D8FFD7}-0.046                                 & \cellcolor[HTML]{D8FFD7}-0.014                                 & \cellcolor[HTML]{D8FFD7}-0.034                                 & \cellcolor[HTML]{D8FFD7}0.002                                  & \cellcolor[HTML]{D8FFD7}-0.006                                 & \cellcolor[HTML]{D8FFD7}-0.011                                 & \cellcolor[HTML]{D8FFD7}-0.058                                 & \cellcolor[HTML]{D8FFD7}-0.018                          & \cellcolor[HTML]{D8FFD7}-0.022                          & \cellcolor[HTML]{D8FFD7}-0.059                        \\
%                                   &                     & \cellcolor[HTML]{ECF4FF}0.183                      & \cellcolor[HTML]{ECF4FF}0.148                               & \cellcolor[HTML]{ECF4FF}0.143                               & \cellcolor[HTML]{ECF4FF}0.156                               & \cellcolor[HTML]{ECF4FF}0.004          & \cellcolor[HTML]{ECF4FF}0.378          & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}0.330   & \cellcolor[HTML]{ECF4FF}0.122          & \cellcolor[HTML]{ECF4FF}0.456 &                     & \cellcolor[HTML]{ECF4FF}0.124          & \cellcolor[HTML]{ECF4FF}0.188          & \cellcolor[HTML]{ECF4FF}0.104          & \cellcolor[HTML]{ECF4FF}0.147          & \cellcolor[HTML]{ECF4FF}inv            & \cellcolor[HTML]{ECF4FF}0.387          & \cellcolor[HTML]{ECF4FF}0.027          & \cellcolor[HTML]{ECF4FF}0.133          & \cellcolor[HTML]{ECF4FF}0.227   & \cellcolor[HTML]{ECF4FF}0.165   & \cellcolor[HTML]{ECF4FF}0.438 \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}0.028                      & \cellcolor[HTML]{FFFFC7}0.074                               & \cellcolor[HTML]{FFFFC7}0.023                               & \cellcolor[HTML]{FFFFC7}0.030                               & \cellcolor[HTML]{FFFFC7}0.003          & \cellcolor[HTML]{FFFFC7}0.058          & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}0.051   & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.054 &                     & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.055          & \cellcolor[HTML]{FFFFC7}0.012          & \cellcolor[HTML]{FFFFC7}0.029          & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}0.058          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.035   & \cellcolor[HTML]{FFFFC7}0.031   & \cellcolor[HTML]{FFFFC7}0.047 \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}0.036                      & \cellcolor[HTML]{EFEFEF}0.041                               & \cellcolor[HTML]{EFEFEF}0.037                               & \cellcolor[HTML]{EFEFEF}0.030                               & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}0.044   & \cellcolor[HTML]{EFEFEF}0.038          & \cellcolor[HTML]{EFEFEF}lose  &                     & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}0.025          & \cellcolor[HTML]{EFEFEF}0.013          & \cellcolor[HTML]{EFEFEF}0.024          & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}0.037   & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}lose  \\
% \multirow{-10}{*}{\rotatebox[origin=c]{90}{\textbf{Adult Census}}}   & \multirow{-5}{*}{X} & \cellcolor[HTML]{FFE2E1}0.055                      & \cellcolor[HTML]{FFE2E1}0.064                               & \cellcolor[HTML]{FFE2E1}0.047                               & \cellcolor[HTML]{FFE2E1}0.053                               & \cellcolor[HTML]{FFE2E1}0.017          & \cellcolor[HTML]{FFE2E1}0.009          & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}0.066   & \cellcolor[HTML]{FFE2E1}0.056          & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{G} & \cellcolor[HTML]{FFE2E1}0.037          & \cellcolor[HTML]{FFE2E1}0.055          & \cellcolor[HTML]{FFE2E1}0.041          & \cellcolor[HTML]{FFE2E1}0.050          & \cellcolor[HTML]{FFE2E1}\textbf{0.018} & \cellcolor[HTML]{FFE2E1}0.031          & \cellcolor[HTML]{FFE2E1}0.031          & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}0.063   & \cellcolor[HTML]{FFE2E1}0.053   & \cellcolor[HTML]{FFE2E1}bad   \\ \hline
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}-0.012}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}-0.023}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}-0.001}                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}-0.007}                                 & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}-0.008                                 & \cellcolor[HTML]{D8FFD7}-0.014                                 & \cellcolor[HTML]{D8FFD7}-0.018                          & \cellcolor[HTML]{D8FFD7}-0.034                          & \cellcolor[HTML]{D8FFD7}-0.014                                 & \cellcolor[HTML]{D8FFD7}-0.082                        &                     & \cellcolor[HTML]{D8FFD7}-0.001                                 & \cellcolor[HTML]{D8FFD7}-0.008                                 & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}0.002                                  & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}0.001                                  & \cellcolor[HTML]{D8FFD7}-0.080                                 & \cellcolor[HTML]{D8FFD7}-0.019                                 & \cellcolor[HTML]{D8FFD7}-0.075                          & \cellcolor[HTML]{D8FFD7}-0.072                          & \cellcolor[HTML]{D8FFD7}-0.143                        \\
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}0.103} & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}0.224}          & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}0.031}          & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}0.038}          & \cellcolor[HTML]{ECF4FF}0.000          & \cellcolor[HTML]{ECF4FF}0.210          & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}lose    & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}0.060          & \cellcolor[HTML]{ECF4FF}bad   &                     & \cellcolor[HTML]{ECF4FF}0.158          & \cellcolor[HTML]{ECF4FF}0.236          & \cellcolor[HTML]{ECF4FF}\textbf{0.166} & \cellcolor[HTML]{ECF4FF}\textbf{0.097} & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}\textbf{0.312} & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}0.058          & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}bad   \\
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}0.035} & \cellcolor[HTML]{FFFFC7}bad                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}0.007}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}0.027}          & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}0.065          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.059   & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad   &                     & \cellcolor[HTML]{FFFFC7}0.032          & \cellcolor[HTML]{FFFFC7}0.051          & \cellcolor[HTML]{FFFFC7}\textbf{0.028} & \cellcolor[HTML]{FFFFC7}\textbf{0.021} & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}\textbf{0.053} & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad   \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}lose                       & \cellcolor[HTML]{EFEFEF}bad                                 & \cellcolor[HTML]{EFEFEF}lose                                & \cellcolor[HTML]{EFEFEF}lose                                & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad   &                     & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}\textbf{0.003} & \cellcolor[HTML]{EFEFEF}\textbf{0.012} & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}inv   \\
%                                   & \multirow{-5}{*}{F} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}0.033} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}0.039}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}0.032}          & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}0.032}          & \cellcolor[HTML]{FFE2E1}0.016          & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.020          & \cellcolor[HTML]{FFE2E1}0.045   & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}0.048          & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{X2} & \cellcolor[HTML]{FFE2E1}0.023          & \cellcolor[HTML]{FFE2E1}0.018          & \cellcolor[HTML]{FFE2E1}\textbf{0.026} & \cellcolor[HTML]{FFE2E1}\textbf{0.027} & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}0.025          & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}bad   \\ \cline{2-25} 
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}-0.002}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}0.002}                                  & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}0.007}                                  & \multicolumn{1}{l|}{\cellcolor[HTML]{D8FFD7}0.000}                                  & \cellcolor[HTML]{D8FFD7}-0.001                                 & \cellcolor[HTML]{D8FFD7}-0.007                                 & \cellcolor[HTML]{D8FFD7}-0.019                                 & \cellcolor[HTML]{D8FFD7}-0.021                          & \cellcolor[HTML]{D8FFD7}-0.058                          & \cellcolor[HTML]{D8FFD7}-0.020                                 & \cellcolor[HTML]{D8FFD7}-0.018                        &                     & \cellcolor[HTML]{D8FFD7}-0.003                                 & \cellcolor[HTML]{D8FFD7}-0.007                                 & \cellcolor[HTML]{D8FFD7}0.014                                  & \cellcolor[HTML]{D8FFD7}0.011                                  & \cellcolor[HTML]{D8FFD7}-0.002                                 & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}-0.066                                 & \cellcolor[HTML]{D8FFD7}-0.017                                 & \cellcolor[HTML]{D8FFD7}-0.058                          & \cellcolor[HTML]{D8FFD7}-0.059                          & \cellcolor[HTML]{D8FFD7}-0.104                        \\
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}0.098} & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}\textbf{0.348}} & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}\textbf{0.114}} & \multicolumn{1}{l|}{\cellcolor[HTML]{ECF4FF}\textbf{0.092}} & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}0.222          & \cellcolor[HTML]{ECF4FF}0.174          & \cellcolor[HTML]{ECF4FF}lose    & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}0.135          & \cellcolor[HTML]{ECF4FF}0.183 &                     & \cellcolor[HTML]{ECF4FF}0.010          & \cellcolor[HTML]{ECF4FF}0.069          & \cellcolor[HTML]{ECF4FF}\textbf{0.011} & \cellcolor[HTML]{ECF4FF}\textbf{0.014} & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}\textbf{0.332} & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}bad   \\
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}0.023} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}\textbf{0.062}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}\textbf{0.023}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFC7}\textbf{0.020}} & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}0.042          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}lose    & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad   &                     & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}0.028          & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}\textbf{0.052} & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.046          & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad   \\
%                                   &                     & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}0.021} & \cellcolor[HTML]{EFEFEF}inv                                 & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{0.011}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{0.018}} & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose    & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}lose  &                     & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}inv     & \cellcolor[HTML]{EFEFEF}inv   \\
% \multirow{-10}{*}{\rotatebox[origin=c]{90}{\textbf{Bank Marketing}}} & \multirow{-5}{*}{X} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}0.043} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}\textbf{0.040}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}\textbf{0.043}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFE2E1}\textbf{0.046}} & \cellcolor[HTML]{FFE2E1}-0.001         & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}0.038          & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}0.048          & \cellcolor[HTML]{FFE2E1}0.043 & \multirow{-5}{*}{G} & \cellcolor[HTML]{FFE2E1}0.014          & \cellcolor[HTML]{FFE2E1}0.023          & \cellcolor[HTML]{FFE2E1}\textbf{0.027} & \cellcolor[HTML]{FFE2E1}\textbf{0.025} & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}\textbf{0.017} & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}0.025          & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}bad   \\ \hline
%                                   &                     & \cellcolor[HTML]{D8FFD7}-0.020                                             & \cellcolor[HTML]{D8FFD7}-0.027                                                      & \cellcolor[HTML]{D8FFD7}-0.012                                                      & \cellcolor[HTML]{D8FFD7}-0.012                                                      & \cellcolor[HTML]{D8FFD7}-0.011                                 & \cellcolor[HTML]{D8FFD7}-0.016                                 & \cellcolor[HTML]{D8FFD7}-0.007                                 & \cellcolor[HTML]{D8FFD7}-0.015                          & \cellcolor[HTML]{D8FFD7}-0.023                          & \cellcolor[HTML]{D8FFD7}-0.506                                 & \cellcolor[HTML]{D8FFD7}-0.446                        &                     & \cellcolor[HTML]{D8FFD7}-0.011                                 & \cellcolor[HTML]{D8FFD7}-0.022                                 & \cellcolor[HTML]{D8FFD7}-0.019                                 & \cellcolor[HTML]{D8FFD7}-0.015                                 & \cellcolor[HTML]{D8FFD7}-0.007                                 & \cellcolor[HTML]{D8FFD7}-0.013                                 & \cellcolor[HTML]{D8FFD7}-0.009                                 & \cellcolor[HTML]{D8FFD7}-0.019                                 & \cellcolor[HTML]{D8FFD7}-0.042                          & \cellcolor[HTML]{D8FFD7}-0.475                          & \cellcolor[HTML]{D8FFD7}-0.203                        \\
%                                   &                     & \cellcolor[HTML]{ECF4FF}bad                        & \cellcolor[HTML]{ECF4FF}0.076                               & \cellcolor[HTML]{ECF4FF}lose                                & \cellcolor[HTML]{ECF4FF}0.060                               & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}0.066          & \cellcolor[HTML]{ECF4FF}0.039          & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}0.095   & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}bad   &                     & \cellcolor[HTML]{ECF4FF}0.109          & \cellcolor[HTML]{ECF4FF}0.130          & \cellcolor[HTML]{ECF4FF}0.103          & \cellcolor[HTML]{ECF4FF}0.108          & \cellcolor[HTML]{ECF4FF}0.035          & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}0.085          & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}lose    & \cellcolor[HTML]{ECF4FF}bad   \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}bad                        & \cellcolor[HTML]{FFFFC7}0.052                               & \cellcolor[HTML]{FFFFC7}lose                                & \cellcolor[HTML]{FFFFC7}0.039                               & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}0.044          & \cellcolor[HTML]{FFFFC7}0.025          & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}0.068   & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad   &                     & \cellcolor[HTML]{FFFFC7}0.077          & \cellcolor[HTML]{FFFFC7}0.092          & \cellcolor[HTML]{FFFFC7}0.070          & \cellcolor[HTML]{FFFFC7}0.078          & \cellcolor[HTML]{FFFFC7}0.021          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.056          & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad   \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}0.044                      & \cellcolor[HTML]{EFEFEF}0.062                               & \cellcolor[HTML]{EFEFEF}0.045                               & \cellcolor[HTML]{EFEFEF}0.059                               & \cellcolor[HTML]{EFEFEF}0.033          & \cellcolor[HTML]{EFEFEF}0.054          & \cellcolor[HTML]{EFEFEF}0.042          & \cellcolor[HTML]{EFEFEF}0.011   & \cellcolor[HTML]{EFEFEF}0.064   & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}bad   &                     & \cellcolor[HTML]{EFEFEF}0.101          & \cellcolor[HTML]{EFEFEF}0.101          & \cellcolor[HTML]{EFEFEF}0.101          & \cellcolor[HTML]{EFEFEF}0.081          & \cellcolor[HTML]{EFEFEF}0.068          & \cellcolor[HTML]{EFEFEF}0.039          & \cellcolor[HTML]{EFEFEF}0.039          & \cellcolor[HTML]{EFEFEF}0.075          & \cellcolor[HTML]{EFEFEF}0.107   & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}bad   \\
%                                   & \multirow{-5}{*}{F} & \cellcolor[HTML]{FFE2E1}lose                       & \cellcolor[HTML]{FFE2E1}bad                                 & \cellcolor[HTML]{FFE2E1}lose                                & \cellcolor[HTML]{FFE2E1}lose                                & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}0.044   & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{S} & \cellcolor[HTML]{FFE2E1}0.019          & \cellcolor[HTML]{FFE2E1}0.034          & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.027          & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}0.059   & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}bad   \\ \cline{2-25} 
%                                   &                     & \cellcolor[HTML]{D8FFD7}0.003                                              & \cellcolor[HTML]{D8FFD7}-0.009                                                      & \cellcolor[HTML]{D8FFD7}-0.014                                                      & \cellcolor[HTML]{D8FFD7}-0.017                                                      & \cellcolor[HTML]{D8FFD7}-0.016                                 & \cellcolor[HTML]{D8FFD7}-0.028                                 & \cellcolor[HTML]{D8FFD7}-0.026                                 & \cellcolor[HTML]{D8FFD7}-0.024                          & \cellcolor[HTML]{D8FFD7}-0.043                          & \cellcolor[HTML]{D8FFD7}-0.466                                 & \cellcolor[HTML]{D8FFD7}-0.443                        &                     & \cellcolor[HTML]{D8FFD7}0.001                                  & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}0.010                                  & \cellcolor[HTML]{D8FFD7}-0.005                                 & \cellcolor[HTML]{D8FFD7}0.000                                  & \cellcolor[HTML]{D8FFD7}0.005                                  & \cellcolor[HTML]{D8FFD7}0.009                                  & \cellcolor[HTML]{D8FFD7}0.007                                  & \cellcolor[HTML]{D8FFD7}-0.002                          & \cellcolor[HTML]{D8FFD7}-0.440                          & \cellcolor[HTML]{D8FFD7}-0.420                        \\
%                                   &                     & \cellcolor[HTML]{ECF4FF}\textbf{0.070}             & \cellcolor[HTML]{ECF4FF}0.091                               & \cellcolor[HTML]{ECF4FF}0.119                               & \cellcolor[HTML]{ECF4FF}0.101                               & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}bad            & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}lose  &                     & \cellcolor[HTML]{ECF4FF}\textbf{0.112} & \cellcolor[HTML]{ECF4FF}\textbf{0.104} & \cellcolor[HTML]{ECF4FF}\textbf{0.065} & \cellcolor[HTML]{ECF4FF}0.123          & \cellcolor[HTML]{ECF4FF}0.038          & \cellcolor[HTML]{ECF4FF}\textbf{0.071} & \cellcolor[HTML]{ECF4FF}\textbf{0.046} & \cellcolor[HTML]{ECF4FF}\textbf{0.064} & \cellcolor[HTML]{ECF4FF}0.150   & \cellcolor[HTML]{ECF4FF}lose    & \cellcolor[HTML]{ECF4FF}bad   \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}\textbf{0.050}             & \cellcolor[HTML]{FFFFC7}0.065                               & \cellcolor[HTML]{FFFFC7}0.082                               & \cellcolor[HTML]{FFFFC7}0.069                               & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.060          & \cellcolor[HTML]{FFFFC7}0.048          & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad   &                     & \cellcolor[HTML]{FFFFC7}\textbf{0.072} & \cellcolor[HTML]{FFFFC7}\textbf{0.075} & \cellcolor[HTML]{FFFFC7}\textbf{0.043} & \cellcolor[HTML]{FFFFC7}0.090          & \cellcolor[HTML]{FFFFC7}0.027          & \cellcolor[HTML]{FFFFC7}\textbf{0.047} & \cellcolor[HTML]{FFFFC7}\textbf{0.028} & \cellcolor[HTML]{FFFFC7}\textbf{0.041} & \cellcolor[HTML]{FFFFC7}0.111   & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}bad   \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}\textbf{0.069}             & \cellcolor[HTML]{EFEFEF}0.074                               & \cellcolor[HTML]{EFEFEF}0.073                               & \cellcolor[HTML]{EFEFEF}0.083                               & \cellcolor[HTML]{EFEFEF}0.036          & \cellcolor[HTML]{EFEFEF}0.064          & \cellcolor[HTML]{EFEFEF}0.064          & \cellcolor[HTML]{EFEFEF}0.055   & \cellcolor[HTML]{EFEFEF}0.091   & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}bad   &                     & \cellcolor[HTML]{EFEFEF}\textbf{0.104} & \cellcolor[HTML]{EFEFEF}\textbf{0.080} & \cellcolor[HTML]{EFEFEF}\textbf{0.085} & \cellcolor[HTML]{EFEFEF}0.076          & \cellcolor[HTML]{EFEFEF}0.066          & \cellcolor[HTML]{EFEFEF}\textbf{0.066} & \cellcolor[HTML]{EFEFEF}\textbf{0.066} & \cellcolor[HTML]{EFEFEF}\textbf{0.049} & \cellcolor[HTML]{EFEFEF}0.115   & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}bad   \\
% \multirow{-10}{*}{\rotatebox[origin=c]{90}{\textbf{German Credit}}}  & \multirow{-5}{*}{X1} & \cellcolor[HTML]{FFE2E1}\textbf{0.020}             & \cellcolor[HTML]{FFE2E1}0.020                               & \cellcolor[HTML]{FFE2E1}0.041                               & \cellcolor[HTML]{FFE2E1}0.037                               & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}0.064   & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{K} & \cellcolor[HTML]{FFE2E1}\textbf{0.017} & \cellcolor[HTML]{FFE2E1}\textbf{0.011} & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}0.034          & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}0.065   & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}bad   \\ \hline
%                                   &                     & \cellcolor[HTML]{D8FFD7}-0.098                                             & \cellcolor[HTML]{D8FFD7}-0.130                                                      & \cellcolor[HTML]{D8FFD7}-0.129                                                      & \cellcolor[HTML]{D8FFD7}-0.128                                                      & \cellcolor[HTML]{D8FFD7}-0.014                                 & \cellcolor[HTML]{D8FFD7}-0.166                                 & \cellcolor[HTML]{D8FFD7}-0.021                                 & \cellcolor[HTML]{D8FFD7}-0.157                          & \cellcolor[HTML]{D8FFD7}-0.179                          & \cellcolor[HTML]{D8FFD7}-0.030                                 & \cellcolor[HTML]{D8FFD7}-0.178                        &                     & \cellcolor[HTML]{D8FFD7}-0.035                                 & \cellcolor[HTML]{D8FFD7}-0.076                                 & \cellcolor[HTML]{D8FFD7}-0.136                                 & \cellcolor[HTML]{D8FFD7}-0.126                                 & \cellcolor[HTML]{D8FFD7}0.065                                  & \cellcolor[HTML]{D8FFD7}-0.139                                 & \cellcolor[HTML]{D8FFD7}-0.015                                 & \cellcolor[HTML]{D8FFD7}-0.155                                 & \cellcolor[HTML]{D8FFD7}-0.189                          & \cellcolor[HTML]{D8FFD7}-0.019                          & \cellcolor[HTML]{D8FFD7}-0.165                        \\
%                                   &                     & \cellcolor[HTML]{ECF4FF}1.549                      & \cellcolor[HTML]{ECF4FF}1.864                               & \cellcolor[HTML]{ECF4FF}1.848                               & \cellcolor[HTML]{ECF4FF}1.849                               & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}0.536          & \cellcolor[HTML]{ECF4FF}0.160          & \cellcolor[HTML]{ECF4FF}1.975   & \cellcolor[HTML]{ECF4FF}2.024   & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}2.303 &                     & \cellcolor[HTML]{ECF4FF}0.501          & \cellcolor[HTML]{ECF4FF}0.885          & \cellcolor[HTML]{ECF4FF}1.411          & \cellcolor[HTML]{ECF4FF}1.303          & \cellcolor[HTML]{ECF4FF}\textbf{0.092} & \cellcolor[HTML]{ECF4FF}0.385          & \cellcolor[HTML]{ECF4FF}0.038          & \cellcolor[HTML]{ECF4FF}1.546          & \cellcolor[HTML]{ECF4FF}1.769   & \cellcolor[HTML]{ECF4FF}lose    & \cellcolor[HTML]{ECF4FF}1.991 \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}0.395                      & \cellcolor[HTML]{FFFFC7}0.571                               & \cellcolor[HTML]{FFFFC7}0.551                               & \cellcolor[HTML]{FFFFC7}0.545                               & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.590   & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}0.651 &                     & \cellcolor[HTML]{FFFFC7}0.121          & \cellcolor[HTML]{FFFFC7}0.275          & \cellcolor[HTML]{FFFFC7}0.462          & \cellcolor[HTML]{FFFFC7}0.447          & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.559          & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}lose    & \cellcolor[HTML]{FFFFC7}0.641 \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}0.274                      & \cellcolor[HTML]{EFEFEF}0.404                               & \cellcolor[HTML]{EFEFEF}0.445                               & \cellcolor[HTML]{EFEFEF}0.446                               & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}0.435   & \cellcolor[HTML]{EFEFEF}0.481   & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}bad   &                     & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}\textbf{0.058} & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}0.419          & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}lose    & \cellcolor[HTML]{EFEFEF}0.426 \\
%                                   & \multirow{-5}{*}{R} & \cellcolor[HTML]{FFE2E1}0.477                      & \cellcolor[HTML]{FFE2E1}0.556                               & \cellcolor[HTML]{FFE2E1}0.534                               & \cellcolor[HTML]{FFE2E1}0.601                               & \cellcolor[HTML]{FFE2E1}0.062          & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.133          & \cellcolor[HTML]{FFE2E1}0.583   & \cellcolor[HTML]{FFE2E1}0.618   & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{G} & \cellcolor[HTML]{FFE2E1}0.183          & \cellcolor[HTML]{FFE2E1}0.305          & \cellcolor[HTML]{FFE2E1}0.467          & \cellcolor[HTML]{FFE2E1}0.445          & \cellcolor[HTML]{FFE2E1}\textbf{0.176} & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.081          & \cellcolor[HTML]{FFE2E1}0.533          & \cellcolor[HTML]{FFE2E1}0.568   & \cellcolor[HTML]{FFE2E1}lose    & \cellcolor[HTML]{FFE2E1}bad   \\ \cline{2-25} 
%                                   &                     & \cellcolor[HTML]{D8FFD7}-0.021                                             & \cellcolor[HTML]{D8FFD7}-0.084                                                      & \cellcolor[HTML]{D8FFD7}-0.091                                                      & \cellcolor[HTML]{D8FFD7}0.000                                                       & \cellcolor[HTML]{D8FFD7}-0.007                                 & \cellcolor[HTML]{D8FFD7}-0.159                                 & \cellcolor[HTML]{D8FFD7}0.015                                  & \cellcolor[HTML]{D8FFD7}-0.134                          & \cellcolor[HTML]{D8FFD7}-0.227                          & \cellcolor[HTML]{D8FFD7}0.004                                  & \cellcolor[HTML]{D8FFD7}-0.152                        &                     & \cellcolor[HTML]{D8FFD7}-0.079                                 & \cellcolor[HTML]{D8FFD7}-0.101                                 & \cellcolor[HTML]{D8FFD7}-0.099                                 & \cellcolor[HTML]{D8FFD7}-0.110                                 & \cellcolor[HTML]{D8FFD7}-0.019                                 & \cellcolor[HTML]{D8FFD7}-0.129                                 & \cellcolor[HTML]{D8FFD7}-0.006                                 & \cellcolor[HTML]{D8FFD7}-0.161                                 & \cellcolor[HTML]{D8FFD7}-0.157                          & \cellcolor[HTML]{D8FFD7}-0.009                          & \cellcolor[HTML]{D8FFD7}-0.159                        \\
%                                   &                     & \cellcolor[HTML]{ECF4FF}0.743                      & \cellcolor[HTML]{ECF4FF}1.619                               & \cellcolor[HTML]{ECF4FF}1.673                               & \cellcolor[HTML]{ECF4FF}\textbf{0.149}                      & \cellcolor[HTML]{ECF4FF}0.086          & \cellcolor[HTML]{ECF4FF}0.597          & \cellcolor[HTML]{ECF4FF}\textbf{0.214} & \cellcolor[HTML]{ECF4FF}2.073   & \cellcolor[HTML]{ECF4FF}bad     & \cellcolor[HTML]{ECF4FF}\textbf{0.154} & \cellcolor[HTML]{ECF4FF}2.557 &                     & \cellcolor[HTML]{ECF4FF}1.364          & \cellcolor[HTML]{ECF4FF}1.701          & \cellcolor[HTML]{ECF4FF}1.470          & \cellcolor[HTML]{ECF4FF}1.663          & \cellcolor[HTML]{ECF4FF}lose           & \cellcolor[HTML]{ECF4FF}0.671          & \cellcolor[HTML]{ECF4FF}0.203          & \cellcolor[HTML]{ECF4FF}1.881          & \cellcolor[HTML]{ECF4FF}1.811   & \cellcolor[HTML]{ECF4FF}0.085   & \cellcolor[HTML]{ECF4FF}2.172 \\
%                                   &                     & \cellcolor[HTML]{FFFFC7}0.101                      & \cellcolor[HTML]{FFFFC7}0.552                               & \cellcolor[HTML]{FFFFC7}0.597                               & \cellcolor[HTML]{FFFFC7}\textbf{0.113}                      & \cellcolor[HTML]{FFFFC7}0.063          & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}\textbf{0.007} & \cellcolor[HTML]{FFFFC7}0.664   & \cellcolor[HTML]{FFFFC7}bad     & \cellcolor[HTML]{FFFFC7}inv            & \cellcolor[HTML]{FFFFC7}0.785 &                     & \cellcolor[HTML]{FFFFC7}0.280          & \cellcolor[HTML]{FFFFC7}0.542          & \cellcolor[HTML]{FFFFC7}0.406          & \cellcolor[HTML]{FFFFC7}0.491          & \cellcolor[HTML]{FFFFC7}lose           & \cellcolor[HTML]{FFFFC7}bad            & \cellcolor[HTML]{FFFFC7}0.065          & \cellcolor[HTML]{FFFFC7}0.587          & \cellcolor[HTML]{FFFFC7}0.567   & \cellcolor[HTML]{FFFFC7}lose    & \cellcolor[HTML]{FFFFC7}0.642 \\
%                                   &                     & \cellcolor[HTML]{EFEFEF}bad                        & \cellcolor[HTML]{EFEFEF}0.467                               & \cellcolor[HTML]{EFEFEF}0.557                               & \cellcolor[HTML]{EFEFEF}\textbf{0.021}                      & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}\textbf{0.009} & \cellcolor[HTML]{EFEFEF}0.647   & \cellcolor[HTML]{EFEFEF}bad     & \cellcolor[HTML]{EFEFEF}inv            & \cellcolor[HTML]{EFEFEF}0.623 &                     & \cellcolor[HTML]{EFEFEF}bad            & \cellcolor[HTML]{EFEFEF}0.400          & \cellcolor[HTML]{EFEFEF}0.285          & \cellcolor[HTML]{EFEFEF}0.389          & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}lose           & \cellcolor[HTML]{EFEFEF}0.472          & \cellcolor[HTML]{EFEFEF}0.473   & \cellcolor[HTML]{EFEFEF}lose    & \cellcolor[HTML]{EFEFEF}0.423 \\
% \multirow{-10}{*}{\rotatebox[origin=c]{90}{\textbf{Titanic}}}        & \multirow{-5}{*}{L} & \cellcolor[HTML]{FFE2E1}0.140                      & \cellcolor[HTML]{FFE2E1}0.562                               & \cellcolor[HTML]{FFE2E1}0.632                               & \cellcolor[HTML]{FFE2E1}\textbf{0.179}                      & \cellcolor[HTML]{FFE2E1}0.101          & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}\textbf{0.067} & \cellcolor[HTML]{FFE2E1}0.707   & \cellcolor[HTML]{FFE2E1}bad     & \cellcolor[HTML]{FFE2E1}inv            & \cellcolor[HTML]{FFE2E1}bad   & \multirow{-5}{*}{X} & \cellcolor[HTML]{FFE2E1}0.300          & \cellcolor[HTML]{FFE2E1}0.532          & \cellcolor[HTML]{FFE2E1}0.356          & \cellcolor[HTML]{FFE2E1}0.524          & \cellcolor[HTML]{FFE2E1}lose           & \cellcolor[HTML]{FFE2E1}bad            & \cellcolor[HTML]{FFE2E1}0.174          & \cellcolor[HTML]{FFE2E1}0.560          & \cellcolor[HTML]{FFE2E1}0.585   & \cellcolor[HTML]{FFE2E1}0.036   & \cellcolor[HTML]{FFE2E1}bad   \\ \hline
% \end{tabular}
% \label{tbl:regions}
% \centering

% \scriptsize \* F: Random Forest, X: XGBoost, L: Logistic Regression, S: Support Vector Classifier, K: K-Nearest Neighbors,  G: Gradient Boosting Classifier. bad: bad trade-off region, lose: lose-lose regions, inv: inverted region. Non-bold numbers represent for good trade-off region. Bold numbers represent for win-win region. T1-4: \fairautoml with different objective functions, AS: \as, R: Reweighing, D: DI Remover, A: Adversarial Debiasing, E: Equalized Odds, C: Calibrated Equalized Odds, O: Reject Option Classification. The colors represent for accuracy and fairness metrics.

% \colorbox{cellgreen}{Accuracy (Acc)}
% \colorbox{cellblue}{Disparate Impact (DI)} \colorbox{cellyellow}{Statistical Parity Difference (SPD)} \colorbox{cellgrey}{Equal Opportunity Difference (EOD)} \colorbox{cellpink}{Average Odds Difference (AOD)} 
% \end{table*}

\begin{table*}[t]
\centering
\caption{Trade-off assessment results of \fairautoml, \as, and mitigation techniques}
\setlength{\tabcolsep}{0.45pt}
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\cline{1-14} \cline{16-28}
                         & \textbf{Model}        & \textbf{Metric} & \textbf{T1}                 & \textbf{T2}                         & \textbf{T3}                         & \textbf{T4}                         & \multicolumn{1}{c|}{\textbf{AS}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{D}} & \multicolumn{1}{c|}{\textbf{A}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c|}{\textbf{C}} & \textbf{O} & \textbf{} & \textbf{Model}        & \multicolumn{1}{c|}{\textbf{Metric}} & \multicolumn{1}{c|}{\textbf{T1}} & \multicolumn{1}{c|}{\textbf{T2}} & \multicolumn{1}{c|}{\textbf{T3}} & \multicolumn{1}{c|}{\textbf{T4}} & \multicolumn{1}{c|}{\textbf{AS}} & \multicolumn{1}{c|}{\textbf{R}} & \multicolumn{1}{c|}{\textbf{D}} & \multicolumn{1}{c|}{\textbf{A}} & \multicolumn{1}{c|}{\textbf{E}} & \multicolumn{1}{c|}{\textbf{C}} & \textbf{O} \\ \cline{1-14} \cline{16-28} 
\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Adult Census}}}   & \multirow{5}{*}{RF}   & Acc             & 0.010                       & 0.001                               & 0.005                               & -0.003                              & 0.016                            & 0.009                           & 0.004                           & -0.066                          & -0.006                          & -0.010                          & -0.047     &           & \multirow{5}{*}{LRG}  & Acc                                  & -0.013                           & -0.022                           & -0.009                           & -0.032                           & -0.001                           & -0.056                          & -0.055                          & -0.121                          & -0.057                          & -0.057                          & -0.061     \\
                                          &                       & DI              & \textbf{0.096}              & \textbf{0.011}                      & \textbf{0.118}                      & 0.095                               & \textbf{0.058}                   & \textbf{0.337}                  & inv                             & 0.215                           & 0.292                           & 0.140                           & 0.445      &           &                       & DI                                   & 0.190                            & 0.410                            & 0.212                            & 0.179                            & 0.040                            & 0.569                           & 0.326                           & bad                             & 0.375                           & 0.335                           & 0.318      \\
                                          &                       & SPD             & \textbf{0.023}              & \textbf{0.024}                      & \textbf{0.038}                      & 0.048                               & \textbf{0.016}                   & \textbf{0.055}                  & inv                             & 0.086                           & 0.047                           & 0.028                           & 0.055      &           &                       & SPD                                  & 0.054                            & 0.075                            & 0.029                            & 0.059                            & 0.005                            & 0.097                           & 0.079                           & bad                             & 0.083                           & 0.081                           & 0.072      \\
                                          &                       & EOD             & \textbf{0.019}              & inv                                 & \textbf{0.014}                      & 0.020                               & \textbf{0.008}                   & inv                             & inv                             & bad                             & 0.041                           & 0.012                           & lose       &           &                       & EOD                                  & 0.048                            & 0.020                            & 0.044                            & 0.049                            & lose                             & 0.057                           & 0.056                           & bad                             & 0.067                           & 0.060                           & 0.059      \\
                                          &                       & AOD             & \textbf{0.028}              & inv                                 & \textbf{0.030}                      & 0.035                               & \textbf{0.021}                   & \textbf{0.005}                  & \textbf{0.001}                  & 0.044                           & 0.051                           & 0.048                           & bad        &           &                       & AOD                                  & 0.085                            & 0.075                            & 0.079                            & 0.089                            & 0.039                            & 0.096                           & 0.094                           & bad                             & 0.103                           & 0.100                           & 0.095      \\ \cline{2-14} \cline{16-28} 
                                          & \multirow{5}{*}{XGB}  & Acc             & -0.019                      & -0.052                              & -0.017                              & -0.015                              & -0.001                           & -0.001                          & -0.018                          & -0.207                          & -0.035                          & -0.035                          & -0.056     &           & \multirow{5}{*}{GBC}  & Acc                                  & -0.023                           & -0.046                           & -0.014                           & -0.034                           & 0.002                            & -0.006                          & -0.011                          & -0.058                          & -0.018                          & -0.022                          & -0.059     \\
                                          &                       & DI              & 0.183                       & 0.148                               & 0.143                               & 0.156                               & 0.004                            & 0.378                           & lose                            & bad                             & 0.330                           & 0.122                           & 0.456      &           &                       & DI                                   & 0.124                            & 0.188                            & 0.104                            & 0.147                            & inv                              & 0.387                           & 0.027                           & 0.133                           & 0.227                           & 0.165                           & 0.438      \\
                                          &                       & SPD             & 0.028                       & 0.074                               & 0.023                               & 0.030                               & 0.003                            & 0.058                           & lose                            & bad                             & 0.051                           & bad                             & 0.054      &           &                       & SPD                                  & bad                              & 0.055                            & 0.012                            & 0.029                            & inv                              & 0.058                           & bad                             & bad                             & 0.035                           & 0.031                           & 0.047      \\
                                          &                       & EOD             & 0.036                       & 0.041                               & 0.037                               & 0.030                               & lose                             & lose                            & lose                            & bad                             & 0.044                           & 0.038                           & lose       &           &                       & EOD                                  & bad                              & 0.025                            & 0.013                            & 0.024                            & inv                              & lose                            & lose                            & lose                            & 0.037                           & bad                             & lose       \\
                                          &                       & AOD             & 0.055                       & 0.064                               & 0.047                               & 0.053                               & 0.017                            & 0.009                           & lose                            & bad                             & 0.066                           & 0.056                           & bad        &           &                       & AOD                                  & 0.037                            & 0.055                            & 0.041                            & 0.050                            & \textbf{0.018}                   & 0.031                           & 0.031                           & lose                            & 0.063                           & 0.053                           & bad        \\ \cline{1-14} \cline{16-28} 
\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Bank Marketing}}} & \multirow{5}{*}{RF}   & Acc             & \multicolumn{1}{l|}{-0.012} & \multicolumn{1}{l|}{-0.023}         & \multicolumn{1}{l|}{-0.001}         & \multicolumn{1}{l|}{-0.007}         & 0.000                            & -0.008                          & -0.014                          & -0.018                          & -0.034                          & -0.014                          & -0.082     &           & \multirow{5}{*}{XGB2} & Acc                                  & -0.001                           & -0.008                           & 0.000                            & 0.002                            & 0.000                            & 0.001                           & -0.080                          & -0.019                          & -0.075                          & -0.072                          & -0.143     \\
                                          &                       & DI              & \multicolumn{1}{l|}{0.103}  & \multicolumn{1}{l|}{0.224}          & \multicolumn{1}{l|}{0.031}          & \multicolumn{1}{l|}{0.038}          & 0.000                            & 0.210                           & lose                            & lose                            & bad                             & 0.060                           & bad        &           &                       & DI                                   & 0.158                            & 0.236                            & \textbf{0.166}                   & \textbf{0.097}                   & lose                             & \textbf{0.312}                  & bad                             & 0.058                           & bad                             & bad                             & bad        \\
                                          &                       & SPD             & \multicolumn{1}{l|}{0.035}  & bad                                 & \multicolumn{1}{l|}{0.007}          & \multicolumn{1}{l|}{0.027}          & lose                             & 0.065                           & bad                             & 0.059                           & bad                             & bad                             & bad        &           &                       & SPD                                  & 0.032                            & 0.051                            & \textbf{0.028}                   & \textbf{0.021}                   & lose                             & \textbf{0.053}                  & bad                             & bad                             & bad                             & bad                             & bad        \\
                                          &                       & EOD             & lose                        & bad                                 & lose                                & lose                                & lose                             & lose                            & lose                            & bad                             & bad                             & lose                            & bad        &           &                       & EOD                                  & lose                             & lose                             & \textbf{0.003}                   & \textbf{0.012}                   & lose                             & inv                             & inv                             & lose                            & bad                             & bad                             & inv        \\
                                          &                       & AOD             & \multicolumn{1}{l|}{0.033}  & \multicolumn{1}{l|}{0.039}          & \multicolumn{1}{l|}{0.032}          & \multicolumn{1}{l|}{0.032}          & 0.016                            & bad                             & 0.020                           & 0.045                           & bad                             & 0.048                           & bad        &           &                       & AOD                                  & 0.023                            & 0.018                            & \textbf{0.026}                   & \textbf{0.027}                   & lose                             & inv                             & inv                             & 0.025                           & bad                             & bad                             & bad        \\ \cline{2-14} \cline{16-28} 
                                          & \multirow{5}{*}{XGB1} & Acc             & \multicolumn{1}{l|}{-0.002} & \multicolumn{1}{l|}{0.002}          & \multicolumn{1}{l|}{0.007}          & \multicolumn{1}{l|}{0.000}          & -0.001                           & -0.007                          & -0.019                          & -0.021                          & -0.058                          & -0.020                          & -0.018     &           & \multirow{5}{*}{GBC}  & Acc                                  & -0.003                           & -0.007                           & 0.014                            & 0.011                            & -0.002                           & 0.000                           & -0.066                          & -0.017                          & -0.058                          & -0.059                          & -0.104     \\
                                          &                       & DI              & \multicolumn{1}{l|}{0.098}  & \multicolumn{1}{l|}{\textbf{0.348}} & \multicolumn{1}{l|}{\textbf{0.114}} & \multicolumn{1}{l|}{\textbf{0.092}} & lose                             & 0.222                           & 0.174                           & lose                            & bad                             & 0.135                           & 0.183      &           &                       & DI                                   & 0.010                            & 0.069                            & \textbf{0.011}                   & \textbf{0.014}                   & lose                             & \textbf{0.332}                  & bad                             & lose                            & bad                             & bad                             & bad        \\
                                          &                       & SPD             & \multicolumn{1}{l|}{0.023}  & \multicolumn{1}{l|}{\textbf{0.062}} & \multicolumn{1}{l|}{\textbf{0.023}} & \multicolumn{1}{l|}{\textbf{0.020}} & lose                             & 0.042                           & bad                             & lose                            & bad                             & bad                             & bad        &           &                       & SPD                                  & lose                             & 0.028                            & inv                              & inv                              & lose                             & \textbf{0.052}                  & bad                             & 0.046                           & bad                             & bad                             & bad        \\
                                          &                       & EOD             & \multicolumn{1}{l|}{0.021}  & inv                                 & \multicolumn{1}{l|}{\textbf{0.011}} & \multicolumn{1}{l|}{\textbf{0.018}} & lose                             & lose                            & lose                            & lose                            & bad                             & bad                             & lose       &           &                       & EOD                                  & lose                             & lose                             & inv                              & inv                              & lose                             & inv                             & lose                            & lose                            & bad                             & inv                             & inv        \\
                                          &                       & AOD             & \multicolumn{1}{l|}{0.043}  & \multicolumn{1}{l|}{\textbf{0.040}} & \multicolumn{1}{l|}{\textbf{0.043}} & \multicolumn{1}{l|}{\textbf{0.046}} & lose                           & lose                            & 0.038                           & lose                            & bad                             & 0.048                           & 0.043      &           &                       & AOD                                  & 0.014                            & 0.023                            & \textbf{0.027}                   & \textbf{0.025}                   & lose                             & \textbf{0.017}                  & lose                            & 0.025                           & bad                             & bad                             & bad        \\ \cline{1-14} \cline{16-28} 
\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{German Credit}}}  & \multirow{5}{*}{RF}   & Acc             & -0.020                      & -0.027                              & -0.012                              & -0.012                              & -0.011                           & -0.016                          & -0.007                          & -0.015                          & -0.023                          & -0.506                          & -0.446     &           & \multirow{5}{*}{SVC}  & Acc                                  & -0.011                           & -0.022                           & -0.019                           & -0.015                           & -0.007                           & -0.013                          & -0.009                          & -0.019                          & -0.042                          & -0.475                          & -0.203     \\
                                          &                       & DI              & bad                         & 0.076                               & lose                                & 0.060                               & lose                             & 0.066                           & 0.039                           & bad                             & 0.095                           & lose                            & bad        &           &                       & DI                                   & 0.109                            & 0.130                            & 0.103                            & 0.108                            & 0.035                            & bad                             & bad                             & 0.085                           & bad                             & lose                            & bad        \\
                                          &                       & SPD             & bad                         & 0.052                               & lose                                & 0.039                               & lose                             & 0.044                           & 0.025                           & bad                             & 0.068                           & bad                             & bad        &           &                       & SPD                                  & 0.077                            & 0.092                            & 0.070                            & 0.078                            & 0.021                            & bad                             & bad                             & 0.056                           & bad                             & bad                             & bad        \\
                                          &                       & EOD             & 0.044                       & 0.062                               & 0.045                               & 0.059                               & 0.033                            & 0.054                           & 0.042                           & 0.011                           & 0.064                           & bad                             & bad        &           &                       & EOD                                  & 0.101                            & 0.101                            & 0.101                            & 0.081                            & 0.068                            & 0.039                           & 0.039                           & 0.075                           & 0.107                           & bad                             & bad        \\
                                          &                       & AOD             & lose                        & bad                                 & lose                                & lose                                & lose                             & lose                            & lose                            & lose                            & 0.044                           & lose                            & bad        &           &                       & AOD                                  & 0.019                            & 0.034                            & bad                              & 0.027                            & lose                             & lose                            & lose                            & lose                            & 0.059                           & lose                            & bad        \\ \cline{2-14} \cline{16-28} 
                                          & \multirow{5}{*}{XGB}  & Acc             & 0.003                       & -0.009                              & -0.014                              & -0.017                              & -0.016                           & -0.028                          & -0.026                          & -0.024                          & -0.043                          & -0.466                          & -0.443     &           & \multirow{5}{*}{KNN}  & Acc                                  & 0.001                            & 0.000                            & 0.010                            & -0.005                           & 0.000                            & 0.005                           & 0.009                           & 0.007                           & -0.002                          & -0.440                          & -0.420     \\
                                          &                       & DI              & \textbf{0.070}              & 0.091                               & 0.119                               & 0.101                               & bad                              & bad                             & bad                             & bad                             & bad                             & lose                            & lose       &           &                       & DI                                   & \textbf{0.112}                   & \textbf{0.104}                   & \textbf{0.065}                   & 0.123                            & 0.038                            & \textbf{0.071}                  & \textbf{0.046}                  & \textbf{0.064}                  & 0.150                           & lose                            & bad        \\
                                          &                       & SPD             & \textbf{0.050}              & 0.065                               & 0.082                               & 0.069                               & bad                              & 0.060                           & 0.048                           & bad                             & bad                             & bad                             & bad        &           &                       & SPD                                  & \textbf{0.072}                   & \textbf{0.075}                   & \textbf{0.043}                   & 0.090                            & 0.027                            & \textbf{0.047}                  & \textbf{0.028}                  & \textbf{0.041}                  & 0.111                           & bad                             & bad        \\
                                          &                       & EOD             & \textbf{0.069}              & 0.074                               & 0.073                               & 0.083                               & 0.036                            & 0.064                           & 0.064                           & 0.055                           & 0.091                           & bad                             & bad        &           &                       & EOD                                  & \textbf{0.104}                   & \textbf{0.080}                   & \textbf{0.085}                   & 0.076                            & 0.066                            & \textbf{0.066}                  & \textbf{0.066}                  & \textbf{0.049}                  & 0.115                           & bad                             & bad        \\
                                          &                       & AOD             & \textbf{0.020}              & 0.020                               & 0.041                               & 0.037                               & lose                             & bad                             & bad                             & lose                            & 0.064                           & bad                             & bad        &           &                       & AOD                                  & \textbf{0.017}                   & \textbf{0.011}                   & inv                              & 0.034                            & lose                             & inv                             & inv                             & inv                             & 0.065                           & lose                            & bad        \\ \cline{1-14} \cline{16-28} 
\multirow{10}{*}{\rotatebox[origin=c]{90}{\textbf{Titanic}}}       & \multirow{5}{*}{RF}   & Acc             & -0.098                      & -0.130                              & -0.129                              & -0.128                              & -0.014                           & -0.166                          & -0.021                          & -0.157                          & -0.179                          & -0.030                          & -0.178     &           & \multirow{5}{*}{GBC}  & Acc                                  & -0.035                           & -0.076                           & -0.136                           & -0.126                           & 0.065                            & -0.139                          & -0.015                          & -0.155                          & -0.189                          & -0.019                          & -0.165     \\
                                          &                       & DI              & 1.549                       & 1.864                               & 1.848                               & 1.849                               & lose                             & 0.536                           & 0.160                           & 1.975                           & 2.024                           & lose                            & 2.303      &           &                       & DI                                   & 0.501                            & 0.885                            & 1.411                            & 1.303                            & \textbf{0.092}                   & 0.385                           & 0.038                           & 1.546                           & 1.769                           & lose                            & 1.991      \\
                                          &                       & SPD             & 0.395                       & 0.571                               & 0.551                               & 0.545                               & lose                             & bad                             & bad                             & 0.590                           & bad                             & lose                            & 0.651      &           &                       & SPD                                  & 0.121                            & 0.275                            & 0.462                            & 0.447                            & inv                              & bad                             & bad                             & 0.559                           & bad                             & lose                            & 0.641      \\
                                          &                       & EOD             & 0.274                       & 0.404                               & 0.445                               & 0.446                               & lose                             & lose                            & lose                            & 0.435                           & 0.481                           & lose                            & bad        &           &                       & EOD                                  & bad                              & bad                              & bad                              & bad                              & \textbf{0.058}                   & lose                            & lose                            & 0.419                           & bad                             & lose                            & 0.426      \\
                                          &                       & AOD             & 0.477                       & 0.556                               & 0.534                               & 0.601                               & 0.062                            & bad                             & 0.133                           & 0.583                           & 0.618                           & lose                            & bad        &           &                       & AOD                                  & 0.183                            & 0.305                            & 0.467                            & 0.445                            & \textbf{0.176}                   & bad                             & 0.081                           & 0.533                           & 0.568                           & lose                            & bad        \\ \cline{2-14} \cline{16-28} 
                                          & \multirow{5}{*}{LRG}  & Acc             & -0.021                      & -0.084                              & -0.091                              & 0.000                               & -0.007                           & -0.159                          & 0.015                           & -0.134                          & -0.227                          & 0.004                           & -0.152     &           & \multirow{5}{*}{XGB}  & Acc                                  & -0.079                           & -0.101                           & -0.099                           & -0.110                           & -0.019                           & -0.129                          & -0.006                          & -0.161                          & -0.157                          & -0.009                          & -0.159     \\
                                          &                       & DI              & 0.743                       & 1.619                               & 1.673                               & \textbf{0.149}                      & 0.086                            & 0.597                           & \textbf{0.214}                  & 2.073                           & bad                             & \textbf{0.154}                  & 2.557      &           &                       & DI                                   & 1.364                            & 1.701                            & 1.470                            & 1.663                            & lose                             & 0.671                           & 0.203                           & 1.881                           & 1.811                           & 0.085                           & 2.172      \\
                                          &                       & SPD             & 0.101                       & 0.552                               & 0.597                               & \textbf{0.113}                      & 0.063                            & bad                             & \textbf{0.007}                  & 0.664                           & bad                             & inv                             & 0.785      &           &                       & SPD                                  & 0.280                            & 0.542                            & 0.406                            & 0.491                            & lose                             & bad                             & 0.065                           & 0.587                           & 0.567                           & lose                            & 0.642      \\
                                          &                       & EOD             & bad                         & 0.467                               & 0.557                               & \textbf{0.021}                      & lose                             & lose                            & \textbf{0.009}                  & 0.647                           & bad                             & inv                             & 0.623      &           &                       & EOD                                  & bad                              & 0.400                            & 0.285                            & 0.389                            & lose                             & lose                            & lose                            & 0.472                           & 0.473                           & lose                            & 0.423      \\
                                          &                       & AOD             & 0.140                       & 0.562                               & 0.632                               & \textbf{0.179}                      & 0.101                            & bad                             & \textbf{0.067}                  & 0.707                           & bad                             & inv                             & bad        &           &                       & AOD                                  & 0.300                            & 0.532                            & 0.356                            & 0.524                            & lose                             & bad                             & 0.174                           & 0.560                           & 0.585                           & 0.036                           & bad        \\ \cline{1-14} \cline{16-28} 
\end{tabular}
\label{tbl:regions}
\centering

\footnotesize \* RF: Random Forest, XGB: XGBoost, LRG: Logistic Regression, SVC: Support Vector Classifier, KNN: K-Nearest Neighbors,  GBC: Gradient Boosting Classifier. bad: bad trade-off region, lose: lose-lose regions, inv: inverted region. Non-bold numbers represent for good trade-off region. Bold numbers represent for win-win region. T1, T2, T3, T4: \fairautoml with different objective functions, AS: \as, R: Reweighing, D: DI Remover, A: Adversarial Debiasing, E: Equalized Odds, C: Calibrated Equalized Odds, O: Reject Option Classification
\end{table*}






==> introduction/problem.tex <==
\section{Preliminaries and problem statement}
\label{sec:problem}


==> introduction/related.tex <==
\section{Related Work}
\label{sec:related}
\subsubsection{AutoML} 
AutoML is a process that improves the efficiency of ML by building a well-performing model architecture for a predictive task. Recently, several AutoML systems have been proposed, which provide both experts and non-experts with a variety of capabilities. For instance, Auto-WEKA~\cite{thornton2013auto} aims to automate constructing models and tuning hyperparameters. TPOT~\cite{olson2016evaluation, olson2016automating} utilizes evolutionary programming to automatically optimize the entire ML pipeline. Auto-Keras~\cite{jin2019auto} utilizes network morphism~\cite{DBLP:journals/corr/ChenGS15, wei2016network} to accelerate the process of tuning neural network. 
Our tool is built on top Scikit-learn \as~\cite{feurer2015efficient}, which uses Bayesian optimization to auto-tune the hyperparameters. \as applies meta-learning and ensemble upgrades to improve efficiency and robustness. 
Currently, the goal of these AutoML tools is tuning the hyperparameter to maximize the accuracy; however, \fairautoml is proposed to repair unfair models.


\subsubsection{Automated Program Repair} 
Automated program repair techniques aim to help developers to accelerate bug fixing process in software. Numerous recent bug repair systems have succeeded in repairing real-life bugs, such as model-based patch ranking~\cite{long2016automatic}, genetic programming~\cite{le2011genprog}, fix
clustering~\cite{bader2019getafix}, patch learning from examples~\cite{bader2019getafix, long2017automatic}, and tree-based edit scripts and patterns~\cite{koyuncu2020fixminer, rolim2017learning, rolim2018learning}. Unlike prior works, \fairautoml utilizes the power of AutoML to fix fairness bugs.


% \paragraph{Multiple objective optimization (MOO)}
% MOO is a process that optimizes systematically and simultaneously several objectives, which can be divided into three categories~\cite{marler2004survey}. The first method is a priori articulation of preferences~\cite{wierzbicki1986methodological, wierzbicki1982mathematical, miettinen2012nonlinear, hwang2012multiple, koski1987norm, ehrgott2003multiobjective} allowing the decision-maker to express their goals of various objectives. The second method that is a posteriori articulation of preferences~\cite{messac2002generating, martinez2001manufacturability, dasimproved, das1998normal, messac2003normalized} is proposed to allow the decision-maker to benefit from selecting preferences from a menu of options. The last one is a method with no articulation of preferences~\cite{hwang2012multiple, zeleny2012multiple,stadler1988fundamentals, hwang1993new, davis2012game, nash1950bargaining, rao1991modified, rao1987game}, which do not necessitate for preferences expression because it is used in the case that the users are unable to express apparently what they desire. In this work, \fairautoml applies the weighted sum method, a method with a priori articulation of preferences, to simultaneously guide AutoML to optimize fairness and accuracy.
% Kamiran \etal~\cite{kamiran2012data} proposed a method to reduce bias by allocating different weights to various groups depending degree of favoritism of a group. 
\subsubsection{Bias mitigation techniques}
Various bias mitigation techniques have been proposed to increase fairness in ML softwares. For instance, Disparate impact remover~\cite{feldman2015certifying} is a pre-processing bias mitigation tool, which edits feature values to decrease bias. Recent methods aim to reduce bias by modifying the ML models throughout the training process, such as adversarial debiasing or prejudice remover regularizer. Adversarial debiasing~\cite{zhang2018mitigating} changes the ML model by providing backward feedback to predict the favourable attribute. Direct prejudice occurs when an ML model makes a decision based on the protected characteristic. Prejudice remover regularizer~\cite{kamishima2012fairness} removes the protected attribute or regulates the effect in the ML model. These works have significantly reduced bias; however, they do not generalize in various datasets/metrics like \fairautoml. 
% The machine learning community has defined different fairness criteria and proposed metrics to measure the fairness of classification tasks . Following the measurement of fairness in ML models, many mitigation techniques have also been proposed to remove bias [15, 19, 22, 25, 29, 32, 41,43, 55, 72, 75]. This body of work mostly concentrates on the theoretical aspect of fairness in a single classification task. Recently, software engineering community has also focused on the fairness in ML, mostly on fairness testing [3, 27, 66, 67]. These works propose methods to generate appropriate test data inputs for the model and prediction on those inputs characterizes fairness. Some research has been conducted to build automated tools [2, 64, 67] and libraries [8] for fairness. In addition, empirical studies have been conducted to compare, contrast between fairness aspects, interventions, tradeoffs, developers concerns, and human aspects of fairness [10, 26, 33, 35, 77].

% \subsection{Search space pruning.}



